Loop ensembles in Stochastic Series Expansion of Two-Dimensional Heisenberg Antiferromagnets

The Stochastic Series Expansion (SSE) method along with resummation over the spin or flavor values maps the partition function of a quantum antiferromagnet to a closely-packed loop gas model in one higher dimension. Earlier work by Nahum et al. has shown that certain closely-packed three-dimensional loop gas models exhibit phases dominated by macroscopic loops, wherein the corresponding joint distribution of loop lengths is Poisson-Dirichlet. On grounds of universality, the same is expected of the ensemble of loops obtained in (2+1)-dimensional quantum antiferromagnets, albeit the loops emerge from a different microscopic origin. We sample the SSE loop ensemble for SU(N) antiferromagnets on a square lattice using Monte Carlo and study how the joint distribution varies with the degree of representation N and inverse temperature $\beta$. We observe that, for low temperatures and small N($\leq$ 4), the distribution indeed shows characteristics of Poisson-Dirichlet behaviour when antiferromagnetic correlations dominate the system.

==> Chapters/AppSim.tex <==
\chapter{Details of simulations}
\section{Computing loop observables in SSE}

In the Stochastic Series Expansion technique, we compute quantities of interest by sampling \textit{configurations} according to their weight in the partition function. Fig.(\ref{SSE_config}) illustrates one such possible configuration for a one-dimensional system. In our work we are concerned only with bipartite lattices. A configuration consists of a state $\ket{\alpha}$ and a string of bond operators that generate a sequence of states by acting on at most one bond.  


A configuration with $M$ time slices consists of an initial basis state ($t=0$) of the lattice, built using $\ket{\pm z}$ at each site, and a sequence of propagated states ($t>0$). Each consecutive state differs from the previous one by atmost one bond. 



\begin{figure}
    \centering
    \includegraphics[width=0.45\columnwidth]{images_new/SSE_config.png}
    \caption{Caption}
    \label{SSE_config}
\end{figure}



\section{Jackknife error estimation \& $\chi^2$ curve fitting}
\section{Estimating $p_{\text{link}} (l)$}

\large \textit{In preparation}



% \section{Monte Carlo based resampling}
% \section{Error saturation study}
% \section{Varying M}


==> FrontMatter/certificate.tex <==
\thispagestyle{plain}

% \begin{multicols}{2}
%  \flushleft
%  \includegraphics[width=20mm]{Images/iitkgplogo.jpg}
%  \columnbreak
%  \par
%  Department of \mydep \\
%  Indian Institute of Technology, Kharagpur \\
%  India - 721302
% \end{multicols}

% \vspace{0.5\baselineskip}
% \hrule
% \vspace{3\baselineskip}

\begin{center}
{\Large {\bf \uppercase{Report Approval}}}
\end{center}

\vspace{\baselineskip}

\noindent This report entitled "{\mytitle}" by { \myname} (Roll No. {\myrollno}) is   approved for the degree of {\bf Dual Degree} (B.Tech. \& M.Tech.)


% \noindent This is to certify that we have examined the thesis entitled {\bf \mytitle}, submitted by {\bf \myname}(Roll Number: {\myrollno}) a postgraduate student of {\bf Department of Physics}  in partial fulfillment for the award of degree of \mydegree. We hereby accord our approval of it as a study carried out and presented in a manner required for its acceptance in partial fulfillment for the Post Graduate Degree for which it has been submitted. The thesis has fulfilled all the requirements as per the regulations of the Institute and has reached the standard needed for submission.

\vspace{3\baselineskip}
\begin{flushright}
\begin{minipage}[c]{0.45\textwidth}
\centering
\vspace{0.5\baselineskip}
{\large \bf Examiners} \\
\vspace{4\baselineskip}
\hrule
\flushright{  Prof. Hridis K. Pal} \\
\vspace{\baselineskip}

\vspace{2.5\baselineskip}
\hrule
\flushright{ Prof. Raghunath Chelakkot} \\
\vspace{\baselineskip}

\vspace{2\baselineskip}
\centering
{\large \bf Supervisor}
\vspace{3\baselineskip}
\hrule
\flushright{ Prof. Sumiran Pujari
} \\
\end{minipage}
\end{flushright}
\vspace{\baselineskip}

\noindent
{Date: 19th August 2022} \\
{Place: Mumbai}

==> FrontMatter/declaration.tex <==
\begin{center}
{\Large {\bf \uppercase{Declaration}}}
\end{center}

\vspace{\baselineskip}

I declare that this written submission represents my ideas in my own words and where
others' ideas or words have been included, I have adequately cited and referenced the original
sources.  I also declare that I have adhered to all principles of academic honesty and integrity
and   have   not   misrepresented   or fabricated   or   falsified   any   idea/data/fact/source   in   my submission.  I understand that any violation of the above will be cause for disciplinary action by the Institute and can also evoke  penal action from the sources which have thus not been properly cited or from whom proper permission has not been taken when needed.

\vspace{3\baselineskip}
\begin{flushright}
\begin{minipage}[c]{0.40\textwidth}
\centering
% \vspace{0.5\baselineskip}
% \hrule
% \vspace{0.5\baselineskip}
\flushright{ Vedant R. Motamarri 
\\  170260005}
\end{minipage}
\end{flushright}

\noindent
$19^{\text{th}}$ August 2022

==> FrontMatter/dedication.tex <==
\thispagestyle{empty}

\pagebreak
\hspace{0pt}
\vfill
\centering
Dedicated to \\
my mother \\
\textbf{\dedicationNamea} \\
\vspace{0.2cm}
and \\
my father \\
\textbf{\dedicationNameb}
\vfill
\hspace{0pt}
\pagebreak
